Hierarchically-Structured Open-Vocabulary Indoor Scene Synthesis with Pre-trained Large Language Model

Indoor scene synthesis aims to automatically produce plausible, realistic and diverse 3D indoor scenes, especially given arbitrary user requirements. Recently, the promising generalization ability of pre-trained large language models (LLM) assist in open-vocabulary indoor scene synthesis. However, the challenge lies in converting the LLM-generated outputs into reasonable and physically feasible scene layouts. In this paper, we propose to generate hierarchically structured scene descriptions with LLM and then compute the scene layouts. Specifically, we train a hierarchy-aware network to infer the fine-grained relative positions between objects and design a divide-and-conquer optimization to solve for scene layouts. The advantages of using hierarchically structured scene representation are two-fold. First, the hierarchical structure provides a rough grounding for object arrangement, which alleviates contradictory placements with dense relations and enhances the generalization ability of the network to infer fine-grained placements. Second, it naturally supports the divide-and-conquer optimization, by first arranging the sub-scenes and then the entire scene, to more effectively solve for a feasible layout. We conduct extensive comparison experiments and ablation studies with both qualitative and quantitative evaluations to validate the effectiveness of our key designs with the hierarchically structured scene representation. Our approach can generate more reasonable scene layouts while better aligned with the user requirements and LLM descriptions. We also present open-vocabulary scene synthesis and interactive scene design results to show the strength of our approach in the applications.

==> CameraReady/Figures/align.tex <==
\begin{figure}
\centering
\includegraphics[width=1\linewidth]{CameraReady/Figures/alignment.pdf}
\caption{Eight possible alignment cases.}
\label{fig:alignment}
\end{figure}

==> CameraReady/Figures/failure_case.tex <==
\begin{figure*}[t]
\centering
\includegraphics[width=\linewidth]{CameraReady/Figures/failure_case_image.pdf}
\caption{Failure cases of our approach.}
\label{fig:failure_case}
\end{figure*}

==> CameraReady/Figures/more_comparison.tex <==
\begin{figure*}[t]
\centering
\includegraphics[width=\linewidth]{CameraReady/Figures/more_comparison_image.pdf}
\caption{More comparison results generated from different approaches.}
\label{fig:more_comparison}
\end{figure*}

==> CameraReady/Figures/more_scene_diversity.tex <==
\begin{figure*}
\centering
\includegraphics[width=\linewidth]{CameraReady/Figures/more_scene_diversity_image.pdf}
\caption{More diverse scenes generated in the open-vocabulary synthesis task.}
\label{fig:more_scene_diversity}
\end{figure*}

==> CameraReady/Figures/more_scene_edit.tex <==
\begin{figure*}
\centering
\includegraphics[width=\linewidth]{CameraReady/Figures/more_scene_edit_image.pdf}
\caption{More language-guided interactive scene editing results.}
\label{fig:more_scene_edit}
\end{figure*}
% 我们的方法可以理解用户需求，并完成场景编辑

==> CameraReady/Figures/prompt_1.tex <==
\begin{figure*}
\centering
\includegraphics[width=\linewidth]{CameraReady/Figures/prompt_1_image.pdf}
\includegraphics[width=\linewidth]{CameraReady/Figures/example_1.pdf}
\caption{Prompt of LLM to generate the hierarchical structure with textual descriptions.}
\label{fig:prompt_1}
\end{figure*}

==> CameraReady/Figures/prompt_2.tex <==
\begin{figure*}
\centering
\includegraphics[width=\linewidth]{CameraReady/Figures/prompt_2_image.pdf}
\includegraphics[width=\linewidth]{CameraReady/Figures/example_2.pdf}
\caption{Prompt of LLM for scene editing.}
\label{fig:prompt_2}
\end{figure*}

==> CameraReady/Figures/user_study_1.tex <==
\begin{figure*}
\centering
\includegraphics[width=\linewidth]{CameraReady/Figures/user_study_1_image.png}
\caption{User interface of perceptual study.}
\label{fig:user study 1}
\end{figure*}

==> CameraReady/Figures/user_study_2.tex <==
\begin{figure*}
\centering
\includegraphics[width=\linewidth]{CameraReady/Figures/user_study_2_image.png}
\caption{User interface of perceptual study.}
\label{fig:user study 2}
\end{figure*}
